WMRB: Learning to Rank in a Scalable Batch Training Approach

We propose a new learning to rank algorithm, named Weighted Margin-Rank Batch loss (WMRB), to extend the popular Weighted Approximate-Rank Pairwise loss (WARP). WMRB uses a new rank estimator and an efficient batch training algorithm. The approach allows more accurate item rank approximation and explicit utilization of parallel computation to accelerate training. In three item recommendation tasks, WMRB consistently outperforms WARP and other baselines. Moreover, WMRB shows clear time efficiency advantages as data scale increases.

==> prelim.tex <==
\section{Introduction}
Rank based learning algorithms have been widely applied to recommendation problems. One prominent example is Weighted Approximate-Rank Pairwise loss \cite{weston2010large}. It aims to achieve a high precision on the \textit{top} of a predicted ranked list instead of an \textit{averaged} high precision over the entire list. However, it is not scalable to extremely large item candidate set in practice due to its intrinsic online learning fashion. %rank-sensitive algorithms are often slow and hard to scale up due to the difficulty of estimating item ranks from an extremely large candidate set. 
%It helps achieve a high precision on the top of a predicted ranked list instead of an averaged high precision over the entire list, as is often preferred.
%In implicit recommendation tasks, people often prefer a high precision on the top of a predicted ranked list instead of an averaged high precision over the entire list.  People  However, it is very challenging  to develop rank-sensitive algorithm partly due to extremely large item candidate set. 
In this work, we addresses the challenge by proposing a batch training approach and empirically demonstrate its advantages in both accuracy and time efficiency.


%In ranking problems such as recommendation and information retrieval, people often prefer a high precision on the top of a predicted ranked list instead of an averaged high precision over the entire list. Popular rank based algorithm BPR~\cite{rendle2009bpr,rendle2014improving} becomes inadequate as it takes mean of the pairwise classification loss.


\section{Background}
%\subsection{Notation}
\textbf{Notation.} Let x denote a user, y an item, and \textbf{Y} the entire item set. $\textbf{y}_x$ denotes items interacted by user x. $\bar{\textbf{y}}_x\equiv\textbf{Y} \setminus \textbf{y}_x$ is the irrelevant item set. We omit x when there is no ambiguity. $f_y(x)$ denotes the model score for user x and item y. 
. The rank of item y is defined as 
\begin{equation}
\label{eq:rank}
r_y = rank_y(f,x,\textbf{y}) =\sum_{\bar{y}\in\bar{\textbf{y}}} \textbf{I}[f_y(x) \le f_{\bar{y}}(x)],
\end{equation}
where \textbf{I} is the indicator function. % is usually approximated by a continuous margin loss $|1-f_y(x) + f_{\bar{y}}(x)|_+$.
Finally, $|t|_+ \equiv max(t,0)$.
%The indicator function is denoted \textbf{I}.  

\textbf{Weighted Approximate-Rank Pairwise loss}
%OWA offers a framework to aggregate the loss non-evenly but it is still computationally expensive to estimate and optimize the loss. 
(WARP) develops an \textit{online} approximation of item ranks. Its critical component is \textbf{an iterative sampling approximation procedure}:
%\begin{itemize}
For each user-item pair (x, y) , sample $y'\in\textbf{Y}$ uniformly with replacement until $1+f_{y'}(x)<f_y(x)$ is violated.
%\end{itemize}
%optimize the top part of a ranked list. However, it is challenging to compute the rank when item set becomes large.
It estimates item ranks by

\begin{equation}
\label{eq:warp3}
r_y\approx rank^{warp}_y(f,x,\textbf{y}) = \lfloor \frac{|\textbf{Y}|-1}{N} \rfloor
\end{equation}
where N is the sampling times to find the violating example. It then incurs a rank sensitive loss weighted by Order Weighted Average~\cite{yager1988ordered}, i.e.,

\begin{equation}
\label{eq:owa}
%\label{eq:alpha}
\Phi^{owa}(r_y) = \sum_{j=1}^{r_y} \alpha_j \quad \alpha_1\ge \alpha_2\ge..\ge 0,
\end{equation}
where decreasing $\alpha$ values control the loss sensitivity to ranks.

\begin{comment}
\section{Notation and Formulation}
In the rest of the paper, x, y denote a user, an item respectively. \textbf{Y} denotes the entire item set. $\textbf{y}_x$ denotes items interacted by user x. $\bar{\textbf{y}}_x\equiv\textbf{Y} \setminus \textbf{y}_x$ is the irrelevant item set. We omit x when there is no ambiguity. The indicator function is denoted \textbf{I}.   $f_y(x)$ denotes the model score for user x and item y. The rank of item y is defined as 
\begin{equation}
\label{eq:rank}
rank_y(f,x,\textbf{y}) =\sum_{\bar{y}\in\bar{\textbf{y}}} \textbf{I}[f_y(x) \le f_{\bar{y}}(x)],
\end{equation}
where the indicator function is usually approximated by a continuous margin loss $|1-f_y(x) + f_{\bar{y}}(x)|_+$. Finally, $|t|_+ \equiv max(t,0)$.

%, y denote an item, bold characters \textbf{y} denote sequences. Normal fonts and subscript indices like $y_j$ denote the j-th element of the corresponding sequence \textbf{y}. $\textbf{Y}$ denotes entire item set and $\bar{\textbf{y}}\equiv\textbf{Y} \setminus \textbf{y}$. 


\section{Preliminary}
\label{sec:background}

\subsection{Ordered Weighted Average}
In implicit recommendation tasks, people often prefer a high precision on the top of a predicted ranked list instead of an averaged high precision over the entire list. To this end, the popular rank based loss BPR~\cite{rendle2009bpr,rendle2014improving} becomes inadequate as it takes mean of the pairwise classification loss. Ordered Weighted Average of classification loss (OWA)~\cite{yager1988ordered}~addresses this by devising a loss that depends on item ranks:

\begin{equation}
\label{eq:owc}
%L = \sum_{(x,\textbf{y})\in S} \sum_{y\in\textbf{y}} L(x,y) = \sum_{(x,\textbf{y})\in S} \sum_{y\in\textbf{y}}\Phi[rank_y(f,x,\textbf{y})]
L^{owa}(x,y) = \Phi^{owa}[rank_y(f,x,\textbf{y})]
\end{equation}
%\sum_{y\in\textbf{y}}

where there exists $\alpha_j$ $j=1,2,..$ such that:
\begin{equation}
\label{eq:alpha}
\Phi^{owa}(k) = \sum_{j=1}^k \alpha_j \quad \alpha_1\ge \alpha_2\ge..\ge 0.
\end{equation}

The function $\Phi^{owa}$ defines a penalty incurred by placing k irrelevant elements before a relevant one. Choosing equal $\alpha_j$ means optimizing the mean rank while choosing $\alpha_{j>1}=0, \alpha_1=1$ means optimizing the proportion of top-ranked correct items. With larger values in the top list of $\alpha$s, it optimizes the top part of a ranked list.

% \subsubsection{Weighted Approximate-Rank Pairwise loss}
\subsection{Weighted Approximate-Rank Pairwise loss}
\label{sec:warp}
OWA offers a framework to aggregate the loss non-evenly but it is still computationally expensive to estimate and optimize the loss. \cite{weston2010large} devised an online approximation and optimization algorithm (WARP) to address this challenge. The critical component of WARP is \textbf{an iterative sampling approximation procedure}:
%\begin{itemize}
For each user-item pair (x, y) , sample $y'\in\textbf{Y}$ uniformly with replacement until $1+f_{y'}(x)<f_y(x)$ is violated.
%\end{itemize}
%optimize the top part of a ranked list. However, it is challenging to compute the rank when item set becomes large.

With the sampling procedure it estimates item ranks by

\begin{equation}
\label{eq:warp3}
rank_y\approx rank^{warp}_y(f,x,\textbf{y}) = \lfloor \frac{|\textbf{Y}|-1}{N} \rfloor
\end{equation}
where N is the sampling times to find the violating example. Given that it approximates the loss with a pairwise loss estimator
% is   It first relaxed indicator function and added a margin to make the loss continuous.
%
%\begin{equation}
%\label{eq:warp1}
%L^1(x,y) = \sum_{i\ne y} \Phi[rank^1_y(f,x,\textbf{y})] \frac{|1-f_y(x) + f_i(x)|_+}{rank^1_y(f,x,\textbf{y})}
%\end{equation}

%Given the violating sample, the error is approximated by 
%an unbiased estimator of the error function $L^1 = \sum_{(x,\textbf{y})\in S} \sum_{y\in\textbf{y}} L^1(x,y)$ is obtained by uniformly sampling (x, y) and a negative item $\bar{y}$, such that it violates $1 + f_{\bar{y}}(x) < f_{y}(x)$,

\begin{equation}
\label{eq:warp2}
\hat{L}^{warp}(x, y) = \Phi^{owa}[rank^{warp}_y(f,x,\textbf{y})] |1-f_y(x) + f_{y'}(x)|_+,
\end{equation}
where the hinge loss also enables (sub)gradient methods during training.

% \subsection{Cross-Entropy Classification loss}
% Cross-entropy classification loss (CE) has been recently exploited in item recommendation~\cite{hidasi2015session,covington2016deep}. For each (x, y) pair, probability of a positive item $y$ is computed
% %\begin{equation}
% %\label{eq:prob}
% as $P_y(f,x,\textbf{y}) = \frac{\exp{f_y(x)}}{\sum_{y'\in \textbf{Y}} \exp{f_{y'}(x)}}$.
% %\end{equation}
% When $|\textbf{Y}|$ is large, the denominator is replaced by a sampled estimator.  Then it incurs the loss,
% \begin{align}
% \label{eq:ce}
% L^{ce}(x,y) &= - \log P_y(f,x,\textbf{y}) = -f_y(x) + \log(\sum_{y'\in \textbf{Y}} \exp{f_{y'}(x)})%\\
% %&= (f_{y^m}(x) - f_{y}(x)) + \log(\sum_{y'\in \textbf{Y} } \exp{(f_{y'}(x)-f_{y^m}(x))})
% \end{align}

% During the training, a batch of items are involved and updated at each iteration.
% %The first term is non-negative. The loss is minimized when $y=y^m$ and $f_y(x)$ is much larger than $f_y'(x)$ for any $y'$. Roughly speaking, CE is close to OWC with $\alpha_1=1, \alpha_{j>0}=0$. 

\end{comment}

==> related.tex <==
\section{Related Work}
\label{sec:related}

Batch training is explored recently to scale up item recommendation. \cite{song2016multi} uses softmax to train a structured deep model on news recommendation.  \cite{covington2016deep} integrates sampled classification losses together with a two-stage classification paradigm to train on YouTube videos recommendation. Logistic loss is used in the ranking stage. \cite{hidasi2015session}~develops new batch losses that take ranking into consideration. Compared to ours, losses in~\cite{hidasi2015session}~only focus on the proportion of top-ranked items.
